Deep Residual Network for Joint Demosaicing and Super-Resolution

In digital photography, two image restoration tasks have been studied extensively and resolved independently: demosaicing and super-resolution. Both these tasks are related to resolution limitations of the camera. Performing super-resolution on a demosaiced images simply exacerbates the artifacts introduced by demosaicing. In this paper, we show that such accumulation of errors can be easily averted by jointly performing demosaicing and super-resolution. To this end, we propose a deep residual network for learning an end-to-end mapping between Bayer images and high-resolution images. By training on high-quality samples, our deep residual demosaicing and super-resolution network is able to recover high-quality super-resolved images from low-resolution Bayer mosaics in a single step without producing the artifacts common to such processing when the two operations are done separately. We perform extensive experiments to show that our deep residual network achieves demosaiced and super-resolved images that are superior to the state-of-the-art both qualitatively and in terms of PSNR and SSIM metrics.

==> texinput/old_copy_.tex <==
\begin{comment}
%\input{texinput/figureIntro2}


There is a growing interest in capturing high-resolution images with increasing quality of the camera sensors and display devices. Despite large advancement in quality of images captured by mobile devices, compact sensors and lenses of the devices limit the resolution. This limitation comes from two sides: the single CCD array of sensors in most of the cameras only measures a subset of red, green, and blue values instead of a full RGB field, and the limited number of pixels of the compact cameras. The former limitation is solved by demosaicing algorithms in the imaging system, while the latter one is usually issued by a post-process of super-resolution.

In the past decades, demoaicing and super-resolution have been studied independently and applied sequentially. However, the separate application of demoaicing and super-resolution is sub-optimal and may leads to error accumulation because artifacts such as color zippering introduced by demosaicing algorithm will be considered as part of the signal in the super-resolution algorithm. As most of the super-resolution algorithms \cite{Dong:2014vh} have assumption that human eyes are more sensitive to the details in the luminance channel than the details in chroma channels, they only deal with noise in luminance channel, which neglect the artifacts in chroma channels caused by demoaicing algorithms. Applying these super-resolution algorithms after demoaicing algorithm may cause visually disturbing artifacts in the end (see examples in Figure. \ref{fig:intro}).
% noise: cite some paper?

Both demosaicing and super-resolution refer to the limitation of the camera, it is reasonable to address them in a unified context. As both of the problems are highly ill-posed due to the loss of the high-frequency information because of the limited sensor, traditional methods explore the missing information among multiple aliased images. Farsiu et al. \cite{Farsiu:2006ug} use a maximum a posteriori approach to estimate the motions between neighboring frames as to improve the rendered resolution of the original Bayer patterns. More recently, Heinze et al. \cite{Heinze:2012vj} proposed a data-driven way of solving this, their method is based on an artificial neural network that gives out high-quality outputs. However, their algorithms lie on the assumptions that small shifts exist between source frames. As the geometry of the single-image and multiframe demosaicing problems are fundamentally different\cite{Farsiu:2006ug}, they cannot deal with single images.

Having assumption that much of high-frequency data is redundant and can be reconstructed from low frequency components, we propose a data-driven framework for joint demosaicing and super-resolution for single image. We build our method on the success of convolutional neural networks (CNN) in many image restoration problems, such as demosaicing \cite{Durand:2016tz}, denoising \cite{Zhang:2017eh}, super-resolution \cite{Dong:2014vh}, etc. These prior works have demonstrate the flexibility of deep CNNs to learn the non-linear relationships between distorted and original images that CNNs not only have less computational cost, but also obtain superior reconstruction accuracy compared to the traditional hand-craft methods \cite{Pulli:2014uh}.
% TODO: cite more papers

\subsection{Contributions}
In this paper, contrary to previous works, we propose to use a deep residual network for doing end-to-end joint demosaicing and super-resolution. More specifically, our network can learn end end-to-end mapping between RGGB Bayer pattern and high-resolution color images. This network generalizes to other color filter array (CFA) with just a simple modification of 2 layers of the network. To the best of our knowledge, it is the first attempt for joint demosaicing and super-resolution. Both tasks are jointly optimized through the network, thus the challenging artifacts such as moire and zipping are eliminated. We also demonstrate our approach enables high-quality results than previous work and runs faster. This approach can be extended also for videos, and can also be integrated into the imaging pipeline.
\end{comment}



\begin{comment}
% TODO: for the whole related work: cite papers
\section{Related Work}
The goal of joint demosaicing and super-resolution is to recover a high-resolution image from a low-resolution Bayer pattern. Both demosaicing and super-resolution are well-studied problem. In this section we show the inefficiency of independent solutions for these problems and discuss the obstacles to designing a unified approach for addressing these two common shortcomings of digital cameras.
% TODO: needs explanation

% add more... & their problems
\subsection{Demosaicing}
To reduce production cost, many camera sensors have only one color measurement (red, green, or blue) per pixel\cite{Farsiu:2006ug}, which is achieved by placing a colorfilter array (CFA) in front of the CCDs. The Bayer pattern is a very common example of such a CFA. Demosaicing is the process to recover the full color image from the incomplete color samples output from this kind of image sensor, which is the crucial first steps of most digital camera pipelines.

To solve this problem, early approaches use different interpolations for luminance channel and chrominance channel in spatial domain\cite{Li:2008ic, Wu:hw} or frequency domain\cite{Glotzbach:jm, Alley:2005ez} to fill in the missing pixels. However, these methods exhibit some challenging artifacts, e.g. zippering and false color artifacts. Previous studies adopted post-processing such as median filter\cite{Hirakawa:cy} to mitigate the artifacs. However, these post-processing raises other issues such as blurry.

Advanced works tend to build the demosaicing on the underlying image statistics. These methods rely on techniques ranging from SVM regression to shallow neural network architectures. Heide et al.\cite{Pulli:2014uh} formulate the demosaicing as an image reconstruction problem and embed a non-local natural image prior into an optimization approach to achieve natural results. Klatzer et al.\cite{Klatzer:2016wg} build a variational energy minimization framework to efficiently learn suitable regularization term from training data, thus yield high quality results in the presence of noise. More recently, Gharbi et al.\cite{Durand:2016tz} proposed a deep learning-based demosaicing method to improve the quality of demosaicing by train on a large dataset.

\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{imgs/method/formation.png}
    \caption{Block diagram presenting the assumed image formation model in our model. Where $I^{HR}$ is the intensity distribution of the real scene, $B$, $D$, $F$ present the blurring, downsampling and color-filtering process, $I^{Bayer}$ is the observed Bayer image. The goal of our joint demosaicing and super-resolution is to estimate a high-resolution image $I^{SR}$ from the observed Bayer image $I^{Bayer}$.}
    \label{fig:formation}
\end{figure*}

\subsection{Single Image Super-Resolution}
Single image super-resolution aims to reconstruct a high-resolution image from a single low-resolution image. Traditional interpolation approaches based on sampling theory\cite{Allebach:1996uz, :2001uc} has encountered limitations in producing realistic details. Recent methods\cite{Elad:2010wu, Egiazarian:2015ww} tend to constrain this ill-posed problem by embedding prior knowledge from large datasets. While these data-driven methods were using simple architectures and hard-coded heuristics, and they do not compare favorably with the state-of-the-art.

Inspired by the success of CNN in image classification tasks\cite{Krizhevsky:2012wl}, various CNN architectures have been proposed for single image super-resolution\cite{Dong:2014vh, Kim:2016wv, Mao:2016ti, Kim:2016kv, Dong:2016ek}. By using modern neural network techniques such as skip-connection\cite{mao:2016} and residual blocks\cite{He:2016tt}, these networks alleviate the burden of carrying identity information in the super-resolution network. They have significantly improved the performance of super-resoltion in terms of peak signal-to-noise ratio (PSNR).

Note that almost all super-resolution methods have been designed to increase the resolution of a single channel (monochromatic) image, they usually only focus on the luminance channel in YCbCr colour space as human are more sensitive to luminance changes\cite{Schulter:2015tz}. Thus these methods are sub-optimal as they do not fully exploit the correlation across the color bands, these methods may fail when the color artifacts exist (see example in Figure. \ref{fig:intro}).
\end{comment}

\begin{comment}
\section{Joint Demosaicing and Super-Resolution}
% draw.io

A common image formation model for imaging systems is illustrated in Figure. ~\ref{fig:formation}. In this model, the real world scene $I^{HR}$ is smoothed by a blur kernel which respect to the point spread function of the camera, then it is downsampled by a factor of $r$ and color-filtered by the CMOS to get the observed Bayer image $I_{Bayer}$. Our goal is to provide an approximate inverse operation estimating a high-resolution image $I^{SR} \approx I^{HR}$ given such a low-resolution Bayer image $I^{Bayer}$. In general, $I^{Bayer}$ is a real-valued tensor of size $H \times W \times 1$, while $I^{HR}$ is a tensor of $r\cdot H \times r\cdot W \times 3$. This problem is highly ill-posed as the downsampling and color-filtering are non-invertiable.

To solve this, traditional methods usually design nonlinear filter to incorporate prior heuristics about inter- and intra-channel correlation, as long as exploit intra-image patch similarity. A deep CNN is a better substitution of these methods, as convolutional layers can naturally explore inter- and intra-channel correlation through a large dataset of natural images. Moreover, the exclusive use of a set of convolutional layers enables jointly optimizing all the parameters to minimize a single objective, as being feasible for joint demosaicing and super-resolution.

Thus we build our framework based on data-driven fashion: we create the training set from a large set of high-quality images $I^{HR}$, and produce the input measurements $I^{Bayer}$ using the same process as the mentioned image formation model (illustrated in Figure. ~\ref{fig:formation}), then we train our deep convoluiontal network on this dataset.  

\begin{figure*}[]
    \centering
    \includegraphics[width=.95\linewidth]{imgs/method/network.png}
    \caption{Illustration of our proposed network architecture. The network is a feed-forward fully convolutional network that maps a low-resolution Bayer image to a high-reosolution color image. Conceptually the network has three components: color extraction of Bayer image, non-linear mapping from Bayer image representation to color image representation with feature extraction, and high-resolution color image reconstruction. }
    \label{fig:network}
\end{figure*}

\subsection{Deep Residual Network for Joint Demosaicing and Super-Resolution}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Stage & Layer & Output Shape  \\
        \hline
        \hline
        \multicolumn{2}{|c|}{Input (Bayer image)} &  $h \times w \times 1$ \\
        \hline
        1 & Conv with a stride of 2 & $\frac{h}{2} \times \frac{w}{2} \times C$ \\
          & Sub-pixel Conv & $h \times w \times \frac{C}{4}$ \\
          & Conv, PReLU & $h \times w \times C$\\
        \hline
        2 & Residual Block & $h \times w \times C$ \\
          & ... & $h \times w \times C$  \\
          & Residual Block & $h \times w \times C$  \\
        \hline
        3 & Sub-pixel Conv & $2\cdot h \times 2\cdot w \times \frac{C}{4}$ \\
          & Conv, PReLU & $2\cdot h \times 2\cdot w \times C$ \\
          & Conv & $2\cdot h \times 2\cdot w \times 3$ \\
        \hline
        \multicolumn{2}{|c|}{Output (color image)} & $2\cdot h \times 2\cdot w \times 3$\\
        \hline
    \end{tabular}
    \caption{The summary of our network architecture. The stages are corresponding to the three stages ($1, 2, 3$ present color extraction, feature extraction \& non-linear mapping, reconstruction, respectively) illustrated in Figure.~\ref{fig:network}. We set the number of filters $C = 256$ and use 32 residual blocks in stage 2.}
    \label{tab:network}
\end{table}
We use a standard feed-forward network architecture to implement our joint demosaicing and super-resolution, which is presented in Figure ~\ref{fig:network}. The goal of the network is to recover from $I^{Bayer}$ an image $I^{SR} = F(I^{Bayer})$ that is as similar as possible to the ground truth high-resolution color image $I^{HR}$. We wish to learn a mapping $F$ from a large corpus of images, which conceptually consists of three stages:
\begin{enumerate}
  \item \textbf{Color Extraction:} this operation separate the different color pixels into different channels from the mono-channel Bayer image. With this operation, no hand-crafted rearrangement of the Bayer input is needed as in other demosaicing algorithms~\cite{Durand:2016tz, Pulli:2014uh, Tan:2017}, the network generalizes to different CFAs given different input measurements. This operation gives a set of color features from the Bayer input.
  \item \textbf{Feature Extraction \& Non-linear Mapping:} follow the intuition of building the first deep neural network for super-resolution ~\cite{Dong:2014vh}, this operation extract overlapping patches from the color features to use high-dimension vectors to represent the Bayer image in low-resolution manifold, then maps it to the high-resolution manifold. 
  \item \textbf{Reconstruction:} this operation aggregates high-resolution representations to generate the final high-resolution color image $I^{SR}$.
\end{enumerate}

\subsubsection{Color Extraction}

The Bayer image is a tensor with different color presenting sequentially in one channel. To make the spatial pattern translation invariant and reduces the computational cost in the latter steps, it is essential to separate the colors in Bayer image into different channels at the beginning. Since Bayer pattern is ubiquitous and have a spatial size of $s \times s$, and where $s = 2$ and the neighboring Bayer pattern may also affects color, we build our first convolutional layer $L_{1}$ with a spatial size of $2 \cdot s$ and a stride of $s$:
\begin{equation}
I^{1} = L_{1}(I^{Bayer})_{(x,y)} = (W_1 * I^{Bayer} + b_1)_{(2\cdot x, 2\cdot y)},
\end{equation}
where $I^1$ represents the output from the first layer, $W_1$ and $b_1$ represent the filters and biases of the first convolutional layer, and $*$ denotes the convolution operation. Here, $W_1$ corresponds to $C = 256$ filters of support $2 \cdot s \times 2 \cdot s$.

We build an efficient sub-pixel convolutional Layer~\cite{Shi:2016tm} $L_{2}$ to upsample the color features back to the original resolution:
\begin{equation}
L_{2}(I^{1})_{(x,y,c)}=I^{1}_{(\left \lfloor \frac{x}{s} \right \rfloor, \left \lfloor \frac{y}{s} \right \rfloor, \frac{C \dot mod(y,s)}{s}+\frac{C \cdot mod(x,s)}{s^2}+c)},
\end{equation}
here, the sub-pixel convoluitonal layer is equivalent to a shuffling operation which reshape a tensor of size $H \times W \times C$ into a tensor of size $s \cdot H \times s\cdot W \times \frac{C}{s^2}$. We find that applying this sub-pixel convolutional layer helps reduce checkerboard artifacts in the output.

Due to the linearity of the separation operation, no activation function is utilized in both layers.

% results show in experiments?? 
Note that this color extraction operation can be generalized to other CFAs by modifying $s$ respect to the spatial size of the specific CFA. Thus we have $s = 2$ for all kinds of Bayer filters, CYGM filter or RGBE filter, and $s = 6$ for the X-trans pattern.

\subsubsection{Feature Extraction \& Non-linear Mapping}
\begin{figure}
    \centering
    \includegraphics[width=.95\linewidth]{imgs/method/block.png}
    \caption{Illustration of the architecture of our residual blocks. We remove the batch normalization layer in the original residual blocks ~\cite{He:2016tt} and replace the ReLU with Parametric ReLU ~\cite{He:2015cv}. This structure enables faster convergence and better performance.}
    \label{fig:residual}
\end{figure}
Inspired by Dong et al. ~\cite{Dong:2014vh}, to explore relationships between inside and between channels, as to finally represent the Bayer image in a high-resolution manifold, we exploit a group of convolutional layers in this step.

Previous works ~\cite{He:2016tt} have demonstrated that residual networks exhibits excellent performance both in accuracy and training speed in computer vision problems from the low-level to high-level tasks. We build a set of $n_b$ residual blocks each having a similar architecture as Lim et al. ~\cite{Lim:2017un}, which is demonstrated in Figure. ~\ref{fig:residual}. We remove the batch normalization layers in the original residual blocks ~\cite{He:2016tt} since these layers get rid of range flexibility from networks by normalizing the features ~\cite{Lim:2017un}. We also replace the activation functions ReLU with Parametric ReLU~\cite{He:2015cv}(PReLU) for preventing dead neurons and gradient vanishing caused by ReLU. These modifications helps stabilize training and reduce color shift artifacts in the output. For convenient network setting, we set all residual network with same number of filters as $C = 256$.

\subsubsection{Reconstruction}
In the reconstruction stage, we apply another sub-pixel convolutional layer to upsample the extracted features to the desired resolution, then followed a final convolutional layer to reconstruct the high-resolution color image.
\end{comment}

\section{Conclusion}
In this paper, we propose an efficient framework for joint demosaicing and super-resolution, which is capable of recovering high-quality color images from Bayer mosaics. Our approach does not produce disturbing color artifacts. Our proposed method outperforms the combinations of the state-of-the-art demosaicing algorithms and the state-of-the-art super-resolution algorithms in both quantitative measurements and perceptual quality.
